Document Collection Visual Question Answering

Current tasks and methods in Document Understanding aims to process documents as single elements. However, documents are usually organized in collections (historical records, purchase invoices), that provide context useful for their interpretation. To address this problem, we introduce Document Collection Visual Question Answering (DocCVQA) a new dataset and related task, where questions are posed over a whole collection of document images and the goal is not only to provide the answer to the given question, but also to retrieve the set of documents that contain the information needed to infer the answer. Along with the dataset we propose a new evaluation metric and baselines which provide further insights to the new dataset and task.

==> figs/document_examples.tex <==


\begin{figure}
\centering
\begin{tabular}{p{0.49\textwidth} p{0.49\textwidth}}
% \includegraphics[width=\linewidth, keepaspectratio]{figs/document_examples/doc_0454_super_zoomed_alt.jpg} &
% \includegraphics[width=\linewidth, keepaspectratio]{figs/document_examples/doc_2231_super_zoomed_alt.jpg} \\
\includegraphics[width=\linewidth, keepaspectratio]{figs/document_examples/doc_0454_ultra_zoomed.jpg} &
\includegraphics[width=\linewidth, keepaspectratio]{figs/document_examples/doc_2231_ultra_zoomed.jpg} \\
\multicolumn{2}{l}{Q: In which years did Anna M. Rivers run for the State senator office?} \\
\multicolumn{2}{l}{A: [2016, 2020]} \\
\multicolumn{2}{l}{E: [454, 10901]} \\



% \begin{tabular}{p{0.98\textwidth}}
% \includegraphics[width=\linewidth, keepaspectratio]{figs/doc_0454.jpg} \\
\end{tabular}
\caption{Top: Partial visualization of sample documents in DocCVQA. Bottom: Example question from the sample set, its answer and their evidences. In DocCVQA the evidences are the documents where the answer can be inferred from. In this example, the correct answer are the years 2016 and 2020, and the evidences are the document images with ids 454 and 10901 which corresponds to the forms where Anna M. Rivers presented as a candidate for the State senator office.}
\label{fig:example_docs}
\end{figure}



==> results_section_backup.tex <==
\section{Baselines}

This section describes the baselines that are employed in the experiments. Given the nature of the DocCVQA dataset, we breakdown the task into two different subtasks. First, through a retrieval approach we rank the documents according to the confidence relative to the question. Then, from the documents with the highest confidence, we get the answer to the question.

\subsection{Retrieval}

\subsubsection{Text spotting:}


% Check in other papers if they were writting the Q, D... in italics??
The objective of the text spotting approach is to rank the documents according to a confidence relative to a question. For that, we first run a Part Of Speech (POS) tagger over the question to identify the most relevant words in it by keeping only nouns and digits, and discard the rest of the words. Then, as described in equation \ref{eq:confidence} for each relevant word in the question we get the minimum Levenshtein distance \cite{levenshtein1966binary} between all the words extracted through an OCR in the document and the question word. Then, we average all the distances and use the result as the confidence that the document is relevant to the question.

\begin{equation} \label{eq:confidence}
c = \frac{1}{|Q|} \sum_{q=1}^{Q} \min_{d=1}^{D}(qw_q, dw_d)
\end{equation}


Notice that removing only stopwords is not enough, as for example in the question depicted in figure FIGURE, the verb \emph{run} is not considered as stopword, but can't be found in the document and consequently would be counterproductive.

FIGURE - Pensar si mostro la pregunta aquí explicitament o la integro dins de exemples de imatges i preguntes?

        
% NLTK POS tag.  keep = ['NNS', 'NNP', 'NN', 'CD']
% 'CD': Cardinal Digit, 'NN':Singular Noun, 'NNS':Plural Noun, 'NNP': Proper Noun



\subsubsection{Database approach:}

In the dataset approach, even though it also consist on ranking the documents according to a confidence, in this case the result is binary, pointing out if a document is relevant or not. For that, we first run a commercial OCR over the document collection, extracting not only the recognized text, but also the key-value relationship between the field names and their values, including checkboxes. Once this information has been extracted, we dump everything into a database like data structure. Then, when a question is performed, the fields in the query are compared with those in the stored records. If all the constraints are met, that document is considered relevant and is given a confidence of 1, while otherwise, it is given a confidence of 0.

It is very important to consider two relevant aspects in this baseline. % First, the dump of the key-value information to a database like structure requires of the normalization and correction from the recognized keys-text to the fields names we already know we can find in the forms. This means that this is a very rigid method ....
First, it is a very rigid method that does not allow any modification in the data and therefore, is not generalizable at all. Moreover, it requires of a preprocessing that is currently done manually to parse the query from Natural Language to a Structured Query Language (SQL). Despite these limitations, we consider it is an  interesting baseline because it offers an insight of what would be the performance of such approaches in this dataset.

% Es pot donar més detalls de com es fa el bolcat de dades de strings recognized a BBDD like.

% Es pot incloure en algún lloc, tant aquí com a Conclusions i Future work: 1) Que hi ha un researh field en NLP que consisteix en parsejar una consulta NLP a SQL i 2) Que aquest parsing manual en realitat es pot crear des d'un inici a partir d'un formulari en html.

% Figura mostrant les dades extretes amb Amazon textract

% Fer un experiment del dataset approach sense la neteja?


\subsection{Answering}

\subsubsection{BERT:}
To answer the asked questions over the document collection we make use of BERT \cite{devlin2018bert} question answering model. BERT is a task agnostic language representation based on transformers \cite{vaswani2017attention} that can be afterwards used in other downstream tasks. In our case, we use extractive question answering BERT models which consist on predicting the start and end indices of the answer span from a context, usually a passage or paragraph. Hence, we extract the answer for each of the documents ranked with highest confidence in the retrieval module. Nonetheless, there is not such context in the DocCVQA documents that encompasses all the textual information. Therefore, we follow the approach of \cite{mathew2021docvqa} to build this context by serializing the recognized OCR tokens on the document images to a single string separated by spaces, following a top-left to bottom-right order.


% Explicar que segueix el ranking
%     Explicar thresholds?
    
% Explicar com es crea el context a partir

% els quals consisteixen en proposar la resposta a partir d'un passatge o paragraph.





% Experiments Minesh
% In addition to the VQA models which can read text, we try out extractive question answering / reading comprehension models from NLP. In particular, we use BERT [9] question answering models. BERT is a method of pre-training language representations from unlabelled text using transformers [38]. These pretrained models can then be used for downstream tasks with just an additional output layer. In the case of extractive Question Answering, this is an output layer to predict start and end indices of the answer span

% For QA using BERT, three pre-trained BERT models from the Transformers library [40] are used. The models we use are bert-base-uncased, bert-large-uncasedwhole-word-masking and bert-large-uncased-whole-wordmasking-finetuned-squad. We abbreviate the model names as bert-base, bert-large and bert-large-squad respectively. Among these, bert-large-squad is a pre-trained model which is also finetuned on SQuAD 1.1 for question answering. In case of extractive question answering or reading comprehension datasets ‘contexts’ on which questions are asked are passages of electronic text. But in DocVQA ‘contexts’ are document images. Hence to finetune the BERT QA models on DocVQA we need to prepare the data in SQuAD style format where the answer to a question is a ‘span’ of the context, defined by start and end indices of the answer. To this end we first serialize the OCR tokens recognized on the document images to a single string, separated by space, in top-left to bottom-right order. To approximate the answer spans we follow an approach proposed in TriviaQA [18], which is to find the first match of the answer string in the serialized OCR string.


\subsubsection{Database approach:}
Following this approach, we only need to retrieve the value of the specified field in the query...

\section{Results}
\input{tables/results.tex}




% Retrieval: E
% \input{tables/results_retrieval.tex}
\input{tables/results_all.tex}
